The Clinical Trials Puzzle: How Network Effects Limit Drug Discovery

The depth of knowledge offered by post-genomic medicine has carried the promise of new drugs, and cures for multiple diseases. To explore the degree to which this capability has materialized, we extract meta-data from 356,403 clinical trials spanning four decades, aiming to offer mechanistic insights into the innovation practices in drug discovery. We find that convention dominates over innovation, as over 96% of the recorded trials focus on previously tested drug targets, and the tested drugs target only 12% of the human interactome. If current patterns persist, it would take 170 years to target all druggable proteins. We uncover two network-based fundamental mechanisms that currently limit target discovery: preferential attachment, leading to the repeated exploration of previously targeted proteins; and local network effects, limiting exploration to proteins interacting with highly explored proteins. We build on these insights to develop a quantitative network-based model of drug discovery. We demonstrate that the model is able to accurately recreate the exploration patterns observed in clinical trials. Most importantly, we show that a network-based search strategy can widen the scope of drug discovery by guiding exploration to novel proteins that are part of under explored regions in the human interactome.

==> commented.tex <==
% We extend these works by quantifying innovation from a large corpus of clinical trials encompassing several drugs and diseases. 

% this paper looked at the use of natural products in clinical trial testing \cite{butler2014natural}

% This data has also been provided important information about compliance in reporting , characteristics of trials reported \cite{califf2012characteristics}, and publication impact \cite{chen2016publication}. 


% the focus of this work
%In this work, we quantify drug innovation through the lens of  therapeutic targets, that is, innovative drugs test new proteins in the well defined drug-target network\cite{ay2007drug}, where drug-targets interact with other proteins that can be involved in diseases\cite{menche2015uncovering, guney2016network}. 
% Since the majority of new drugs rely on binding to protein, known as targets\cite{gates2021wealth}, the underlying protein-protein interaction (PPI) network provides an useful bedrock to quantify innovation in clinical trials.

%Interestingly, even Phase 1 trials, whose primarily goal is to establish the target mechanisms for new drugs\cite{ivy2010approaches}, rarely test novel drugs and novel targets (Fig \ref{fig:prop_new_ct} Phase 1). 

%As a result of this preferential attachment, across Phases 1 through 4, 50\% of the trials test previously approved drugs, and only 30\% of the trials test novel compounds, while 20\% of trials test a combination of approved and novel drugs (Fig \ref{fig:prop_new_ct} D). 

%We also find that the number of approved drugs in trials decreases following the end of the patent period for a drug molecule, lasting between 8 to 14 years post approval (Fig \ref{fig:si_approval_num_trials}). 
%Interestingly, new trials of previously approved drugs tend to test diseases different from the FDA approved condition (Fig \ref{fig:si_approval_repurposing}), evidence of drug repurposing efforts in clinical trials. 

%Increased attention of approved drugs in clinical trials, however, leads to ineffective resource allocation, taking away resources from testing new drugs, and can be detrimental to the discovery of novel targets.

\begin{comment}
% practical utility of clinical trials
The past decade has seen an explosion of data mining methods that has been paramount in accelerating the pace of drug discovery \cite{bagherian2021machine,vamathevan2019applications, schneider2020rethinking}. 
Pharmaceutical scientists can now take advantage of a combination of advanced machine learning\cite{cao2013genome,jacob2008protein} (e.g. deep learning) and network science\cite{luo2017network,chen2012drug,zhang2017network} (e.g. graph neural networks) techniques for the identification of potential drug candidates using large-scale pharmacological databases\cite{chen2016drug, brown2017standard}, prompting the emergence of a new field of network medicine\cite{sonawane2019network, barabasi2011network, loscalzo2017network} and network pharmacology\cite{hopkins2008network}, thus greatly reducing the cost of conducting exhaustive experimental testing as a first screening \cite{chong2007new}. Yet, these computational advances are ineffectual if the discovered knowledge about drugs (\textit{in-silico}) is not actively transferred to applied settings (\textit{in-vitro}) by conducting clinical trials on novel targets. 

% has transformed the methods  advancements in network science techniques (e.g. graph neural networks) has also helped in predicting drug-target interactions\cite{luo2017network,chen2012drug,zhang2017network}, drug positioning\cite{wu2013network}, drug combinations\cite{cheng2019network}, and drug repurposing \cite{sadegh2020exploring, gysi2020network}.

%Computational approaches to drug discovery are gaining popularity because they can reliably confirm novel, promising drug candidates experimentally, thereby greatly reduce the cost of conducting exhaustive \textit{in-vitro} testing (i.e. on cells and whole organisms) \cite{chong2007new}. Computational approaches to drug discovery are gaining popularity because they can reliably identify novel and promising drug candidates, without \textit{in-vitro} experimenting, thus greatly reducing the cost of conducting exhaustive experimental testing as a first screening \cite{chong2007new}. While the strides in computational medicine can highlight new opportunities for drugs and significantly speed up the drug-to-market timeline, they are a small piece in the big puzzle of drug development. Although important for advancing drug research, these methods are ineffectual if the knowledge is not actively transferred to applied settings. In other words, clinical trials need to actively test novel candidates for us to reap the benefits of \textit{in-silico} (i.e. virtual screening) drug exploration. But, how innovative are these trials in discovering new treatments? Are clinical trial studies at the forefront of improving our combined knowledge about how the human genome can help us treat diseases and disorders? 

%n general, these techniques either use docking simulations of 3-D structures of genes to identify potential binding sites\cite{cheng2007structure}

% These targets are found to be most useful in the vicinity of the disease genes, also known as the disease module [cite]. 

%\footnote{\url{ http://www.fda.gov/MedicalDevices/DeviceRegulationandGuidance/HowtoMarketYourDevice/PremarketSubmissions/PremarketApprovalPMA/default.htm}}. 

% It is also found that the bio-pharmaceutical industry invests as much as five times more in research and development, relative to their sales, than the average United States (US) manufacturing firm\footnote{Congressional Budget Office (CBO) of the United States 2006 report on pharmaceutical industry. Accessed from: \url{https://www.cbo.gov/sites/default/files/109th-congress-2005-2006/reports/10-02-drugr-d.pdf}. Page 9.}, making clinical trials a big part of the Gross Domestic Product (GDP) of the US. 

% Identifying the drivers of biological innovation in clinical trials will help develop policies that will encourage efficient exploration of protein targets and equitable exploration of diseases. 

% understanding drug target innovation
Estimating scientific value per dollar investment in a clinical trial for a new drug is a challenging task. 
Indeed, innovation potential of a new drug can take several forms, ranging from minor changes in its molecular profile, to increased ability in patients response and minimizing  side-effects\cite{aronson2020me}. 
In a simplistic model, the innovation potential is achieved by drugs that explores novel therapeutic targets, that is, innovative drugs test new proteins in the well defined drug-target network\cite{ay2007drug}, where drug-targets interact with other proteins that can be involved in diseases\cite{menche2015uncovering, guney2016network}. 
Since the majority of new drugs rely on  their protein bind affinity, known as targets\cite{gates2021wealth}, the underlying protein-protein interaction (PPI) network provides an useful bedrock to quantify innovation in clinical trials.
\end{comment}


\begin{comment}
\section*{Conclusion}

In this work, we recreated the exploration patterns of the PPI network in drug discovery by combining open source data from multiple sources, allowing us to examine the underlying forces driving collective discovery of new drugs. We find minimal novelty in clinical trials in that new drugs rarely test novel targets, leading to heavy inequality in target exploration and preferential selection of a few known targets. Further, we find that the proteins tested in trials and the proteins associated to FDA approved drugs are located in close proximity within the PPI network, indicating the valuable role of networks in prompting new drug exploration. We quantify this network effect through a predictive model and find that the likelihood of selecting a protein for a new drug is proportional to the number of drugs tested in its neighborhood.

Finally, we find that the present choices in target selection leads to much lower exploration benefits than expected if proteins were selected at random. Through computational simulations, we show that a network based search process could yield higher exploration benefits. As we move towards novel therapeutics for diseases, clinical design for new drugs may be more complicated, requiring high development costs and increased development timelines. The optimal innovation path may rely not on preferring wider exploration over deeper exploitation but a rewarding combination of both that allows us to utilize the promise of new therapies available in diverse regions of the human genome.

\end{comment}


%We find that proteins associated with disease are three times more likely to be in a clinical trial compared to proteins with no known disease association (Fig \ref{fig:odds_ratio}; Table \ref{tab:reg_results}). However, proteins associated with common diseases are more likely to be associated with a drug than proteins associated with rare diseases (OR: 2.2 [CI: 1.8, 2.7] versus 1.7 [CI: 1.5, 1.8]). 
%Further, proteins experience increased likelihood of becoming the target of a new drug when it in the target of multiple approved drugs (OR: 3.6 [CI: 3.5, 3.7]). For example, when a protein has ten new drug approved, its odds of being the target of a new drug increases almost nine fold. 

%In a similar manner, proteins are more likely to be in a trial if they have been associated with drugs with multiple trials (OR: 1.4 [CI: 1.39, 1.41]). For example, a protein experiences a two-fold increase in the number of experimental drugs targeting it, it becomes 2.6 [CI: 2.5, 2.7] times more likely to be the target of a new drug. These results indicate that the attractiveness of a protein as a drug candidate increases as more drugs and trials begin to focus on it in the clinical pipeline, highlighting the role of increased clinical exposure.

%We find that while interacting with a disease protein decreases the likelihood of exploration (OR: 0.86 [CI: 0.77, 0.97]), a protein interacting both with a disease associated protein and a previously tested protein experiences an increased likelihood of exploration (OR: 1.12 [CI:1.01, 1.25]). That is, drug-target exploration is prevalent for proteins connected to disease associated proteins that have been previously tested rather than proteins part of disease neighborhood with no experimental drugs. 

%Further, increased exploration numbers within a protein's local network increases its likelihood to be selected for a new drug. We find that a two-fold increase in the number of approved drugs in the neighborhood of a protein increases its likelihood to be associated with a new drug (OR: 1.03 [CI: 1.01, 1.05]). In a similar fashion, proteins with an increased number of clinical trials in its neighborhood (OR: 1.02 [CI: 1.01, 1.03]) and proteins embedded in a neighborhood with increased drug exploration experience increased likelihood to be associated to a new drug (OR: 1.02 [CI: 1.01, 1.03]). 

%In other words, the likelihood that a protein will be selected for a new drug depends not only on preferential attachment but also on the exploration patterns of its local neighborhood. 

%These results indicate that a protein located in network neighborhoods with increased exploration receive higher attention as new drug-targets compared to proteins located in network neighborhoods with fewer clinical trials. For example, when a protein has ten new drug approved, its odds of being the target of a new drug increases almost nine fold.

% The choice of targets is situated in the PPI network and improves our collective knowledge about the drug interactions in the human genome. 

% We tease out the network features that may govern drug-target exploration. We find that over time the drug innovation has been accelerated in regions with previously validated targets (\textbf{Fig \ref{fig:ppi_net}}). The targets that were identified of prominence in 1995 (A), upon being successfully verified, has enabled exploration of its neighboring genes in subsequent years (2005 B, 2015 C). Indeed, this is a normal collective discovery behavior in several real-world systems\cite{iacopini2020interacting} where nodes explored in previous times guides future exploration. However, in the case of clinical trials, given the pace of discovery (\textbf{Fig \ref{fig:new_drugs_targets}}), this approach is not a desirable outcome. This leads to over-testing of known drugs and genes, effectively ignoring the inactive parts of the network. There is benefit in conducting multiple trials and creating multiple drugs with targets in the same region, but it comes at a cost of collective discovery. While the investment in drugs and clinical trials has increased over time, we find ourselves with several inactivate regions of the network that are yet to be tested.

% As a consequence to this minimized outlook of the network, a target is more likely to be part of trials if its neighborhood is also actively tested (\textbf{Fig \ref{fig:prop_neighbors_tested}}). We find that across the same time instances of network observation as earlier majority of the targets that are active at that time had 10-20\% of its neighboring genes already in clinical trials (colored All). This is also true for the newly introduced genes at these time periods (colored New). It is true that over time the network would converge to a point where there are no more isolated nodes that has no neighbors tested. However, we find that at these time periods there were/ a lot of available genes that has scarce neighborhood exploration (colored Available). 

\begin{comment}
\textbf{Innovation potential of unbiased drug discovery}

The growing homogeneity in tested targets and the lack of novel drugs in clinical trials, raises the question, can we successfully optimize drug discovery to maximize the diversity in tested targets? We apply our network model to identify drug candidates for three autoimmune diseases - Rheumatoid Arthritis (RA), Crohn Disease (CD), and Asthma. 
We begin by curating the set of disease associated proteins that were already tested in clinical trials, representing the baseline of previously tested proteins. Next, we identify proteins that interact with the tested proteins, mapping the explored network neighborhoods. Utilizing the obtained network, we scan for all possible values of $q$ in three regimes: (i) PA ($p = 0.95$); (ii) R ($p=0.5$); (iii) LN ($p=0.05$); and rank proteins based on the frequency they are targeted. Finally, we use the identified list of druggable proteins\cite{freshour2021integration} as positive samples, and evaluate the model performance by investigating whether the predicted protein has been verified as a potential drug-target, allowing us to have a precision measure. The method is designed to predict drug candidates by searching the neighborhood of disease associated proteins that are part of previous clinical trials.

%text about p and q
We find that a network driven search for drug targets not only improves the diversity in tested targets but also helps identify potential drug candidates (Fig \ref{fig:net_scenarios} H). Specifically, we find that when seeking to reduce preferential attachment ($p=0.05$), increasing the network search parameter from $q=0.05$ to $q=0.95$, can improve target diversity (0 to 1) and provide a 40\% improvement in drug prediction (0.5 to 0.7), and the R strategy finds a 20\% (0.75 to 0.9) in successful drug discovery. Indeed, by preferring to test previously tested targets at high rates ($p=0.95$), the network model always finds druggable targets with high success rates (0.98). However, the PA strategy also consistently tests fewer targets than the R or LN strategies (Fig \ref{fig:net_scenarios} C-E), and also provides low variety in tested targets (Fig \ref{fig:net_scenarios} F), resulting in an overall slower exploration of the human interactome. Taken together, we find that a combined strategy of network oriented search of drug targets and reduction in preferential selection of targets have vast societal benefits with minimal reduction in drug discovery. 

The network model also offers an unbiased exploration strategy, characterized by $TD=0$ (Fig \ref{fig:net_scenarios} F, blue line). This strategy represents the choices ($p$, $q$) that result in an equal number of untargeted proteins part of explored neighborhoods and previously tested proteins are selected as drug targets. That is, under the condition, a new drug is just as likely to target a previously tested protein as it is to target any one of its neighboring proteins that have not yet been tested in clinical trial, representing an unbiased approach to drug discovery. We find that the unbiased exploration strategy selects novel druggable drug candidates with high accuracy (Supplementary Table \ref{tab:novel_drug_candidates}) for RA (Druggable Precision@10: 0.8), CD (Druggable Precision@10: 0.8), and Asthma (Druggable Precision@10: 0.9). Importantly, the model is able to predict drug candidates in the local network neighborhood of disease-associated proteins (Fig \ref{fig:net_scenarios} H). For example, the method selected the protein NLRP3 as a potential drug candidate for both CD and RA. NLRP3 interacts with proteins ABCB1, HSP90AA1, CYP3A4, NR1I2, proteins that have been associated to RA and that were previously tested in clinical trials (Fig \ref{fig:net_scenarios} G, NLRP3). Indeed, mutations downstream of NLRP3 play an essential role in regulating the inflammasome, identified as a risk factor for inflammatory diseases\cite{villani2009common}. Animal model studies verified that the regulating the over-expression of this gene inhibits the maturation of interleukin-1$\beta$ (IL-1$\beta$), and reduces RA-induced inflammation\cite{liu2020cinnamaldehyde}. These results indicate that pursuing an unbiased approach to drug discovery can help improve the target diversity in clinical trials and help identify potential drug candidates, presenting \textit{in-silico} validity of network-driven approaches facilitating unbiased drug discovery.

% Technological progress is inheritably a dynamic process. It is hardly a random process but is the result of the accumulation of inventive and innovative activities over time. In a dynamic setting, competition from new entrants in the market, that experiment with new technologies, has become the driving force for innovation, and in turn market incumbents are forced to innovate for their survival.

% Development and initiation of clinical trials is an expansive process spanning large teams and several years.  
%Given the nature of pharmaceutical companies, they are found to rely heavily on secret endeavors in the hope to claim first movers' advantage, especially in patenting \cite{cohen2000protecting}. 


% We present new strategies to optimize drug exploration patterns, analysis that is useful to both pharmaceutical funders and policy makers alike seeking to allocate resources to improve collective  .

%We observe an increasing trend in the number of new drug trials every year, with over 4,000 new clinical trials, on average, yearly for the past ten years (Fig \ref{fig:ct_counts} A), indicating a monotonous increase in investments from funders for drugs. 


%The first trial usually takes a long time but the targets receive increased quicker attention (time since last drug trial) as the community begins to accept the utility of that target. 
% Given that the targets are inter-connected in the PPI network, do we observe features of networked exploration, where genes associated with other identified, explored targets increases its network visibility? 


% Following the current growth pattern at the onset of 2050, clinical trials would have tested 6256 proteins (33\% of the human genome) and introduced 7846 drugs.\footnote{Calculated by fitting $y = k*x^{bt}$. coefficients obtained from least squares fit- for targets $k = 26.45, bt = 1.27$; drugs: $k = 2.07, bt = 1.91$} 


%\dgnote{on DB you can also see drugs that were withdrawn, it might be a good idea to know how many drugs, even after approved had left market, I think that now there are +- 700 drugs approved - and commercialized.} \kvnote{I see! but that may be going out of scope? because withdrawal of drugs means failed innovation and by our way of thinking that is still innovation right?}


%797 (38\% of all drug-targets) proteins

%Further, we find that proteins tested in clinical trials tend to cluster in the same region of the network (Fig \ref{fig:ppi_net} A, pink nodes), forming a largest connected component consisting of 2,449 proteins (94\% of all targets) (p < 0.001; Supplementary Fig \ref{fig:si_lcc}). The region of proteins targeted by experimental drugs (Fig \ref{fig:ppi_net}, pink nodes), has significant network overlap with the region enriched with proteins that target FDA approved drugs (Fig \ref{fig:ppi_net} A, green nodes), as measured by the network-separation score\cite{menche2015uncovering} ($S_{a,b} = -0.3$, $p <0.001$; Supplementary Fig \ref{fig:si_sep}). The effect persists in high-throughput protein interactions as well ($S_{a,b} = -0.7$, $p<0.001$; Supplementary Fig \ref{fig:si_sep_hiunion}), hence it is not driven by potential selection biases of the PPI. 


%To validate the model's ability to identify potential drug targets, we ask the model to identify drug candidates for three autoimmune diseases - Rheumatoid Arthritis (RA), Crohn Disease (CD), and Asthma. We begin by identifying disease proteins associated to each of the three disease that were tested in previous clinical trials (Supplementary Section 7.2). Next, we search the interaction of these proteins and pick untargeted proteins among them, representing proteins that are part of explored neighborhoods. Next, we use the model to select proteins through the three outlined strategies (PA, R, LN), allowing us to rank proteins based on the frequency they are targeted. Finally, the proteins in the network are validated as druggable, based on extensive experimental studies. We use the widely curated and accepted list of druggable proteins, \cite{freshour2021integration} to investigate whether the predicted protein has been verified as a potential drug-target, allowing us to measure if the exploration pattenrs leads to potential druggable outcomes. We present the results for RA (Fig \ref{fig:net_scenarios} D, E), the similar outcomes for CD and Asthma, being discussed in the Supplementary Section \ref{fig:si_prec_cd_asthma}.

\end{comment}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
